Multicolor Photometry of the Neptune Irregular Satellite Neso

We report on time series photometry of the faint Neptune irregular satellite Neso. Observations in the V, R, and I pass-bands were performed in photometric conditions at the Cerro Paranal observatory using the instrument FORS2, in the night of July 15th, 2010. Astrometry and photometry derived from these observations are presented here. The time coverage of about six hours does not allow to construct a light curve and derive a meaningful rotational period. However, we could derive new estimates of apparent magnitudes obtaining R=25.2 pm 0.2 mag in agreement with Brozovic, Jacobson, Sheppard (2011), and also V=25.6 pm 0.3 mag, and I=24.5 pm 0.3. In this way we could derive for the first time Neso colors, V-I=1.0 pm 0.4 mag, R-I=0.7 pm 0.4 mag and V-R=0.3 pm 0.4 mag. We compared those colors with those in Peixinho, Delsanti, Doressoundiram (2015). The color R-I appears to be slightly redder than the typical values for Centaurs and KBOs, the color V-I is in nice agreement with both populations. The large error-bars prevents from assigning Neso to any of the reference classes, just looking at Neso colors, although the data seem to suggest that we can rule out its membership in classes of resonant objects or Plutinos.

==> Table1.tex <==
\begin{deluxetable}{ccccccc}
\tablecaption{Astrometric and photomeric data for NESO, 2010 July 15\label{tab:1}}
\tablehead{
\colhead{UT} & \colhead{RA(J2000.0)} & \colhead{Dec(J2000.0)} & \colhead{Filter} & \colhead{Airmass} & \colhead{Exp.Time (secs)} & \colhead{Mag}
}
\startdata
02:58:04.455 &  22:01:37.34  &   -12:26:34.87  &    R  &  1.920  &  600  &  25.4 \\
03:08:40.521 &  22:01:37.26  &   -12:26:35.03  &    I  &  1.798  &  600  &  24.1 \\
03:20:20.734 &  22:01:37.33  &   -12:26:34.51  &    V  &  1.683  &  600  &  25.2 \\
03:31:03.481 &  22:01:37.19  &   -12:26:35.58  &    R  &  1.593  &  600  &  25.3 \\
03:41:39.538 &  22:01:37.17  &   -12:26:35.82  &    I  &  1.551  &  300  &  24.8 \\
03:47:05.577 &  22:01:37.14  &   -12:26:35.86  &    I  &  1.513  &  300  &  24.6 \\
03:53:43.412 &  22:01:37.12  &   -12:26:35.96  &    V  &  1.439  &  600  &  25.5 \\
04:04:26.449 &  22:01:37.08  &   -12:26:36.12  &    R  &  1.380  &  600  &  25.2 \\
04:15:02.517 &  22:01:37.06  &   -12:26:36.27  &    I  &  1.352  &  300  &  25.1 \\
04:20:30.705 &  22:01:37.03  &   -12:26:36.40  &    I  &  1.327  &  300  &  25.1 \\
04:27:36.114 &  22:01:36.99  &   -12:26:36.69  &    V  &  1.276  &  600  &  25.7 \\
04:38:18.511 &  22:01:36.95  &   -12:26:36.74  &    R  &  1.236  &  600  &  25.1 \\
04:48:54.437 &  22:01:36.93  &   -12:26:36.93  &    I  &  1.217  &  300  &  24.3 \\
04:54:23.057 &  22:01:36.91  &   -12:26:37.14  &    I  &  1.200  &  300  &  24.4 \\
05:01:18.504 &  22:01:36.84  &   -12:26:40.47  &    V  &  1.166  &  600  &  25.4 \\
05:12:01.492 &  22:01:36.82  &   -12:26:37.47  &    R  &  1.139  &  600  &  24.7 \\
05:22:37.448 &  22:01:36.79  &   -12:26:37.52  &    I  &  1.127  &  300  &  24.3 \\
05:28:05.997 &  22:01:36.78  &   -12:26:37.51  &    I  &  1.115  &  300  &  24.2 \\
05:35:21.816 &  22:01:36.76  &   -12:26:37.61  &    V  &  1.093  &  600  &  25.1 \\
05:46:04.414 &  22:01:36.71  &   -12:26:38.14  &    R  &  1.076  &  300  &  25.0 \\
05:56:40.521 &  22:01:36.69  &   -12:26:38.28  &    I  &  1.068  &  300  &  24.8 \\
06:02:08.589 &  22:01:36.67  &   -12:26:38.12  &    I  &  1.061  &  300  &  24.9 \\
06:08:54.996 &  22:01:36.62  &   -12:26:38.75  &    V  &  1.048  &  600  &  25.3 \\
06:19:37.303 &  22:01:36.59  &   -12:26:38.96  &    R  &  1.039  &  600  &  25.4 \\
06:30:13.530 &  22:01:36.56  &   -12:26:39.23  &    I  &  1.035  &  300  &  24.2 \\
06:35:41.979 &  22:01:36.54  &   -12:26:39.08  &    I  &  1.032  &  300  &  24.0 \\
06:42:27.105 &  22:01:36.52  &   -12:26:39.25  &    V  &  1.026  &  600  &  25.8 \\
06:53:09.383 &  22:01:36.46  &   -12:26:39.55  &    R  &  1.024  &  600  &  25.6 \\
07:03:45.499 &  22:01:36.44  &   -12:26:39.77  &    I  &  1.023  &  300  &  23.8 \\
07:09:13.988 &  22:01:36.42  &   -12:26:39.74  &    I  &  1.023  &  300  &  24.7 \\
07:15:47.623 &  22:01:36.39  &   -12:26:40.03  &    V  &  1.025  &  600  &  25.5 \\
07:26:30.371 &  22:01:36.36  &   -12:26:40.13  &    R  &  1.029  &  600  &  25.3 \\
07:37:06.497 &  22:01:36.32  &   -12:26:40.43  &    I  &  1.031  &  300  &  24.5 \\
07:42:34.687 &  22:01:36.30  &   -12:26:40.45  &    I  &  1.035  &  300  &  24.5 \\
07:49:14.322 &  22:01:36.28  &   -12:26:40.39  &    V  &  1.043  &  600  &  25.6 \\
07:59:57.409 &  22:01:36.29  &   -12:26:40.59  &    R  &  1.054  &  600  &  25.1 \\
08:10:33.617 &  22:01:36.21  &   -12:26:40.92  &    I  &  1.060  &  300  &  24.5 \\
08:16:01.956 &  22:01:36.18  &   -12:26:41.10  &    I  &  1.067  &  300  &  24.5 \\
08:22:41.182 &  22:01:36.15  &   -12:26:41.40  &    V  &  1.084  &  600  &  25.8 \\
08:33:23.428 &  22:01:36.11  &   -12:26:41.45  &    R  &  1.102  &  600  &  25.1 \\
08:43:59.605 &  22:01:36.10  &   -12:26:41.54  &    I  &  1.113  &  300  &  24.5 \\
08:49:28.015 &  22:01:36.06  &   -12:26:41.43  &    I  &  1.124  &  300  &  24.8 \\
08:56:06.490 &  22:01:36.03  &   -12:26:41.81  &    V  &  1.151  &  600  &  25.8 \\
09:06:49.418 &  22:01:35.99  &   -12:26:42.20  &    R  &  1.179  &  600  &  25.3 \\
09:17:25.754 &  22:01:35.97  &   -12:26:42.14  &    I  &  1.196  &  300  &  24.9 \\
09:22:54.244 &  22:01:35.94  &   -12:26:42.55  &    I  &  1.213  &  300  &  24.7 \\
09:29:31.409 &  22:01:35.92  &   -12:26:42.67  &    V  &  1.252  &  600  &  25.9 \\
09:40:14.527 &  22:01:35.87  &   -12:26:42.90  &    R  &  1.294  &  600  &  25.4 \\
09:50:50.793 &  22:01:35.84  &   -12:26:42.78  &    I  &  1.318  &  600  &  24.6 \\
09:56:18.652 &  22:01:35.81  &   -12:26:43.17  &    I  &  1.343  &  600  &  24.6 \\
\enddata
\end{deluxetable}


